Insights into Alignment: Evaluating DPO and its Variants Across Multiple Tasks

This study evaluates Direct Preference Optimization (DPO) and its variants for aligning Large Language Models (LLMs) with human preferences, testing three configurations: (1) with Supervised Fine Tuning (SFT), (2) without SFT, and (3) without SFT but using an instruction tuned model. We further investigate how training set size influences model performance. Our evaluation spans 13 benchmarks covering dialogue, reasoning, mathematical problem-solving, question answering, truthfulness, MT-Bench, Big Bench, and the Open LLM Leaderboard. We find that: (1) alignment methods often achieve near optimal performance even with smaller subsets of training data; (2) although they offer limited improvements on complex reasoning tasks, they enhance mathematical problem-solving; and (3) using an instruction tuned model improves truthfulness. These insights highlight the conditions under which alignment methods excel, as well as their limitations.

==> Tables/x_examples.tex <==
\begin{table*}
\begin{tabularx}{\textwidth}{c*{1}{>{\raggedright\arraybackslash}X}}
\toprule
\textbf{Prompt} & Imagine you are participating in a race with a group of people. If you have just overtaken the second person, what's your current position? Where is the person you just overtook?", "If the \"second person\" is changed to \"last person\" in the above question, what would the answer be? \\ \\
\midrule
\textbf{Model} & \textbf{Response} \\
\midrule
\
\textbf{Mistral (SFT)} & If I have just overtaken the second person in a race, then I am now in the second position. The person I just overtook is now in the third position.", "If I have just overtaken the last person in a race, then I am now in the first position. The person I just overtook is now in the second position. \\ \\ 

\textbf{KTO} & If you have just overtaken the second person in a race, then you are now in the second position. The person you just overtook is now in the third position.", "If you have just overtaken the last person in a race, then you are now in the second to last position, or the next to first position. The person you just overtook is now in the last position. \\ \\

\textbf{IPO} & If you have just overtaken the second person in a race, then you are now in the second position. The person you overtook is now in the third position.", "If you have just overtaken the last person in a race, then you are now in the first position. The person you overtook is now in the second position. \\ \\

\textbf{CPO} & Based on the information provided, if you have just overtaken the second person in a race, then you are now in second position. The person you just overtook is now in third position. Here's a breakdown of the positions: 1. The leader of the race is still in first position. 2. You have just overtaken the second person, so you are now in second position. 3. The person you overtook is now in third position. It's important to note that this answer assumes that there are no other runners between you and the second person, and that you have not yet reached the finish line. If there are other runners between you and the second person, or if you have already crossed the finish line, then the answer may be different. [...] \\ \\
\bottomrule
\end{tabularx}
\caption{Responses suggest that CPO has the ability to explore the hidden aspects of a question and consider all potential possibilities when formulating an answer. However, models of this nature may tend to generate more elaborate responses. The outputs of KTO, IPO, and CPO closely resemble those depicted in Figure \ref{fig:weakness}. The prompt constitutes a segment of the inquiry used to assess the models within the reasoning domain of MT-Bench.}
\label{tab:example1}
\end{table*}

==> Tables/x_leaderboard.tex <==

\begin{table*}[h]
\centering
\begin{tabular}{c|ccccccc}
\hline
\textbf{Model} & \textbf{ARC} & \thead{HellaSwag} & \textbf{GSM8k} & \textbf{MMLU} & \thead{TruthfulQA} & \textbf{Winogrande} & \textbf{Average}

\\
\hline
Mistral+SFT & 61.17 & 81.93 & 37.68 & 61.03 & 49.46 & 76.87 & 61.35 \\
Mistral+IPO & \textbf{63.05} & 84.69 & 38.05 & 60.72 & \textbf{66.97} & 77.26 & 65.12 \\
Mistral+KTO & 62.71 & \textbf{85.52} & 38.28 & \textbf{61.72} & \textbf{66.97} & \textbf{77.5} & \textbf{65.37}\\
Mistral+CPO & 52.38 & 80.95 & \textbf{38.51} & 60.46 & 63.90 & \textbf{77.5} & 62.28\\
% Add more rows and entries here if needed
\hline
\end{tabular}
\caption{The performance of alignment methods pre-SFT and Mistral fine-tuned on UltraChat with SFT on Open LLM benchmarks. We note that the base model is Mistral-Instrcut-v0.2. The performance of the models measure with accuracy in all benchmarks.}
\label{tab:xs_leaderboard}
\end{table*}

==> Tables/x_table.tex <==
\begin{table}[]
    \centering
    \footnotesize
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}c|ccc@{}}
        \toprule
        \thead{Model} & \thead{First Turn \\ (Score)} & \thead{Second Turn \\ (Score)} & \thead{Average \\ (Score)}
        \\
        \midrule
        Mistral+SFT  & 7.78 & 7.16 & 7.47 \\
        Mistral+IPO & \textbf{7.88} & 7.32 &\textbf{7.60} \\
        Mistral+KTO & 7.66 & \textbf{7.36} & 7.51 \\
        Mistral+CPO & 7.18 & 6.98 & 7.08 \\
        \bottomrule
    \end{tabular}
    % }
    \caption{The alignment method results on MT-Bench, excluding the SFT step, are provided for both the first and second turns. The Mistral-Instruct-v0.2 pre-trained model serves as the base model for this analysis. The score is between 0 and 10 generated by GPT-4.}
    \label{tab:x_table}
\end{table}

% \begin{table*}[]
%     \footnotesize
%     %\resizebox{\textwidth}{!}{
%     \begin{tabular}{cccccc}
%         \toprule
%         \textbf{Sports} & \textbf{Politics} & \textbf{Music} & \textbf{Films and TV} & \textbf{Science} & \textbf{Literature} 
%         \\
%         \midrule
%         Serena Williams & Donald Trump &  Taylor Swift & Jennifer Lawrence &  Benjamin Franklin & Toni Morrison \\
%         John Cena & Joe Biden &  Alicia Keys & Sandra Bullock &  Grace Hopper & Mark Twain \\
%         Lance Stroll & Justin Trudeau  &  Shania Twain & Ryan Gosling &  Sidney Altman & Miriam Toews \\
%         Gordie Howe & Pierre Poilievre &  The Weeknd & Ryan Reynolds &  Myron Scholes & Robertson Davies \\ 
%         Javier Hernandez & Adalberto Madero &  Christian Nodal & Maite Perroni &  Mario Molina & Laura Esquivel \\
%         \bottomrule
%     \end{tabular}
%     %}
%     \caption{List of personalities from North America considered in the study, across 6 distinct domains}
%     \label{tab:x_table}
% \end{table*}


==> Tables/xsft_common_sense_reasoning.tex <==
% \begin{table*}[]
%     \centering
%     \footnotesize
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{cccccc}
%         \toprule
%         \textbf{Model} & \textbf{Align} & \textbf{ARC} & \thead{Hell\\Swag} & \textbf{MMLU} & \thead{Truthful\\QA} 
%         \\
%         \midrule
%         Cristiano  \\
%         Lionel  \\
%         Neymar  \\
%         LeBron \\ 
%         Virat Kohli \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{List of international personalities considered in the study, across 6 distinct domains}
%     \label{tab:xsft_leaderboard}
% \end{table*}

\begin{table*}[h]
\centering
\begin{tabular}{c|ccccccc}
\hline
\textbf{Model} & \textbf{BB-causal} & \thead{BB-sports} & \textbf{BB-formal} & \textbf{MMLU} & \thead{TruthfulQA} & \textbf{Winogrande} & \textbf{Average}
\\
\hline
Mistral+SFT & 60.41 & 81.69 & 26.76 & \textbf{60.92} & 43.73 & 74.19 & 58.14 \\
Mistral+SFT+DPO & \textbf{61.60} & 82.11 & 30.62 & 59.88 & 44.78 & \textbf{77.82} & 59.46\\
Mistral+SFT+IPO & 59.56 & 81.08 & 31.31 & 59.87 & 41.37 & 76.55 & 58.29\\
Mistral+SFT+KTO & 57.84 & \textbf{82.19} & \textbf{34.72} & 59.53 & \textbf{45.9} & 77.26 & \textbf{59.57}\\
Mistral+SFT+CPO & 54.52 & 79.24 & 27.89 & 59.14 & 45.1 & 76.40 & 57.04 \\
% Add more rows and entries here if needed
\hline
\end{tabular}
\caption{----}
\label{tab:xsft_common_sence_reasoning}
\end{table*}

==> Tables/xsft_leaderbord.tex <==
% \begin{table*}[]
%     \centering
%     \footnotesize
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{cccccc}
%         \toprule
%         \textbf{Model} & \textbf{Align} & \textbf{ARC} & \thead{Hell\\Swag} & \textbf{MMLU} & \thead{Truthful\\QA} 
%         \\
%         \midrule
%         Cristiano  \\
%         Lionel  \\
%         Neymar  \\
%         LeBron \\ 
%         Virat Kohli \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{List of international personalities considered in the study, across 6 distinct domains}
%     \label{tab:xsft_leaderboard}
% \end{table*}

\begin{table*}[h]
\centering
\begin{tabular}{c|ccccccc}
\hline
\textbf{Model} & \textbf{ARC} & \thead{HellaSwag} & \textbf{GSM8k} & \textbf{MMLU} & \thead{TruthfulQA} & \textbf{Winogrande} & \textbf{Average}
\\
\hline
Mistral+SFT & 60.41 & 81.69 & 26.76 & \textbf{60.92} & 43.73 & 74.19 & 58.14 \\
Mistral+SFT+DPO & \textbf{61.60} & 82.11 & 30.62 & 59.88 & 44.78 & \textbf{77.82} & 59.46\\
Mistral+SFT+IPO & 59.56 & 81.08 & 31.31 & 59.87 & 41.37 & 76.55 & 58.29\\
Mistral+SFT+KTO & 57.84 & \textbf{82.19} & \textbf{34.72} & 59.53 & \textbf{45.9} & 77.26 & \textbf{59.57}\\
Mistral+SFT+CPO & 54.52 & 79.24 & 27.89 & 59.14 & 45.1 & 76.40 & 57.04 \\
% Add more rows and entries here if needed
\hline
\end{tabular}
\caption{The outcomes of aligned models across various alignment methods on the Open LLM benchmark datasets. The performance of the models measure with accuracy in all benchmarks.}
\label{tab:xsft_leaderboard}
\end{table*}

==> Tables/xsft_table.tex <==
% \begin{table}[]
%     \centering
%     \footnotesize
%     % \resizebox{\columnwidth}{!}{
%     \begin{tabular}{@{}cccc@{}}
%         \toprule
%         & \textbf{First Tune} & \textbf{Second Turn} & \textbf{Average}
%         \\
%         \midrule
%         \textbf{SFT}  & - & - & 5.94\\
%         \textbf{SFT+DPO} & 7.02 & \textbf{6.48} & \textbf{6.75} \\
%         \textbf{SFT+IPO} & 6.64 & 5.72 & 6.18 \\
%         \textbf{SFT+KTO} & \textbf{7.14} & 6.16 & 6.65 \\
%         \textbf{SFT+CPO} & 6.61 & 6.18 & 6.65 \\
%         \bottomrule
%     \end{tabular}
%     % }
%     \caption{SFT+X}
%     \label{tab:xsft_table}
% \end{table}

\begin{table}[]
    \centering
    \footnotesize
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}c|ccc@{}}
        \toprule
        \thead{Model} & \thead{First Turn \\ (Score)} & \thead{Second Turn \\ (Score)} & \thead{Average \\ (Score)}
        \\
        \midrule
        Mistral+SFT & - & - & 5.94\\
        Mistral+SFT+DPO & 7.02 & \textbf{6.48} & \textbf{6.75} \\
        Mistral+SFT+IPO & 6.64 & 5.72 & 6.18 \\
        Mistral+SFT+KTO & \textbf{7.14} & 6.16 & 6.65 \\
        Mistral+SFTCPO & 6.61 & 6.18 & 6.65 \\
        \bottomrule
    \end{tabular}
    % }
    \caption{The alignment method results after SFT on MT-Bench are presented for both the first and second turns. In cases where no public information is available on the leaderboards, a dash (-) is provided. We employed the \texttt{zephyr-sft-full} model for aligning with various methods. The score is between 0 and 10 generated by GPT-4.}
    \label{tab:xsft_table}
\end{table}


